WebTestPilot: Agentic End-to-End Web Testing against Natural Language Specification by Inferring Oracles with Symbolized GUI Elements

Visual language model (VLM) agents show great promise in automating end-to-end (E2E) web testing against requirements in natural language. However, the probabilistic nature of language models can have inherent hallucinations. Therefore, given a detected inconsistency between the requirement and the web application, it is hard to distinguish whether it stems from the hallucination or a real application bug. Addressing this issue presents two core technical challenges: the implicit oracle inference challenge, where the agent must act as its own oracle to implicitly decide if the application's behavior is correct without guidance, and the probabilistic inference challenge, where an LLM's inconsistent reasoning undermines its trustworthiness as an oracle. Existing LLM-based approaches fail to capture such implicit oracles, either by treating any page navigation that doesn't crash as a success, or by checking each state in isolation, thus missing bugs dependent on context from prior steps. We introduce WebTestPilot, an LLM-based agent designed to address these challenges. WebTestPilot uses (1) a symbolization layer which detects and symbolizes critical GUI elements on the web application into symbols (i.e., variables) and (2) translates natural language specification into a sequence of steps, each of which is equipped with inferred pre- and post-conditions over the symbols as an oracle. This oracle captures data, temporal, and causal dependencies, enabling the validation of implicit requirements. To advance research in this area, we build a benchmark of bug-injected web apps for evaluating NL-to-E2E testing. The results show that WebTestPilot achieves a task completion rate of 99%, with 96% precision and 96% recall in bug detection, outperforming the best baseline (+70 precision, +27 recall). The agent generalizes across diverse natural language inputs and model scales.

==> tables/real_bugs.tex <==
\begin{table}[ht]
\caption{Real-world bugs detected by \tool, replicated from GitHub issue trackers.}
\label{table:real_bugs}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{13pt}
\begin{tabular}{|l|l|p{8cm}|l|}
\toprule
\textbf{\#} & \textbf{App} & \textbf{Bug Description} & \textbf{Issue} \\
\hline

1 & Bookstack & Importing books over file size limit fails silently without error & \href{https://github.com/BookStackApp/BookStack/issues/5612}{\#5612} \\ \hline
2 & Bookstack & Blank lines disappearing after saving & \href{https://github.com/BookStackApp/BookStack/issues/5344}{\#5344} \\ \hline
3 & Bookstack & Sorting pages & \href{https://github.com/BookStackApp/BookStack/issues/5074}{\#5074} \\ \hline
4 & Bookstack & Internal server error when creating more than one new user & \href{https://github.com/BookStackApp/BookStack/issues/4862}{\#4862} \\ \hline
5 & Bookstack & Page does not scroll to section when clicking on title in navigation & \href{https://github.com/BookStackApp/BookStack/issues/4330}{\#4330} \\ \hline

6 & Indico & Empty calendar when using back button & \href{https://github.com/indico/indico/issues/3499}{\#3499} \\ \hline
7 & Indico & Duplicate results in search & \href{https://github.com/indico/indico/issues/5287}{\#5287} \\ \hline
8 & Indico & Error when trying to send an email notification about a survey & \href{https://github.com/indico/indico/issues/6667}{\#6667} \\ \hline
9 & Indico & Category search results list contains categories that have been previously deleted & \href{https://github.com/indico/indico/issues/5197}{\#5197} \\ \hline

10 & Invoiceninja & Invoice preview does not update after changing ``surcharge'' fields & \href{https://github.com/invoiceninja/invoiceninja/issues/4072}{\#4072} \\ \hline
11 & Invoiceninja & Clicking on a hyperlink opens a test installation page in the ``Invoice Design'' page & \href{https://github.com/invoiceninja/invoiceninja/issues/4896}{\#4896} \\ \hline
12 & Invoiceninja & Customer documents filter is not working & \href{https://github.com/invoiceninja/invoiceninja/issues/11188}{\#11188} \\ \hline
13 & Invoiceninja & The "Last Year" option in reports uses the current year instead of the last year & \href{https://github.com/invoiceninja/invoiceninja/issues/10876}{\#10876} \\ \hline
14 & Invoiceninja & Issue viewing or downloading documents on invoices & \href{https://github.com/invoiceninja/invoiceninja/issues/10317}{\#10317} \\ \hline
15 & Invoiceninja & Can not edit clients & \href{https://github.com/invoiceninja/invoiceninja/issues/9809}{\#9809} \\ \hline
16 & Invoiceninja & Incorrect payment total in statements & \href{https://github.com/invoiceninja/invoiceninja/issues/10769}{\#10769} \\ \hline

17 & Prestashop & ``Configure'' button is missing in Catalog module & \href{https://github.com/PrestaShop/PrestaShop/issues/22170}{\#22170} \\ \hline
18 & Prestashop & Missing reset button in ``Theme \& Logo'' & \href{https://github.com/PrestaShop/PrestaShop/issues/18893}{\#18893} \\ \hline
19 & Prestashop & The ``Close'' button is not working in the ``Upload'' module modal & \href{https://github.com/PrestaShop/PrestaShop/issues/33629}{\#33629} \\ \hline
20 & Prestashop & The ``Upgrade'' button is not visible even though a new version of the module is available & \href{https://github.com/PrestaShop/PrestaShop/issues/32497}{\#32497} \\ \hline
21 & Prestashop & Can not use the back-office, redirect to login page & \href{https://github.com/PrestaShop/PrestaShop/issues/14796}{\#14796} \\ \hline
22 & Prestashop & Incorrectly calculated prices in the cart due to rounding errors & \href{https://github.com/PrestaShop/PrestaShop/issues/25788}{\#25788} \\ \bottomrule

\end{tabular}
\end{table}
